TidalDecode: Fast and Accurate LLM Decoding with Position Persistent Sparse Attention

Large language models (LLMs) have driven significant advancements across diverse NLP tasks, with long-context models gaining prominence for handling extended inputs. However, the expanding key-value (KV) cache size required by Transformer architectures intensifies the memory constraints, particularly during the decoding phase, creating a significant bottleneck. Existing sparse attention mechanisms designed to address this bottleneck have two limitations: (1) they often fail to reliably identify the most relevant tokens for attention, and (2) they overlook the spatial coherence of token selection across consecutive Transformer layers, which can lead to performance degradation and substantial overhead in token selection. This paper introduces TidalDecode, a simple yet effective algorithm and system for fast and accurate LLM decoding through position persistent sparse attention. TidalDecode leverages the spatial coherence of tokens selected by existing sparse attention methods and introduces a few token selection layers that perform full attention to identify the tokens with the highest attention scores, while all other layers perform sparse attention with the pre-selected tokens. This design enables TidalDecode to substantially reduce the overhead of token selection for sparse attention without sacrificing the quality of the generated results. Evaluation on a diverse set of LLMs and tasks shows that TidalDecode closely matches the generative performance of full attention methods while reducing the LLM decoding latency by up to 2.1x.

==> src/figs/performance/needle/needle_10K_100K.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{c c c c c c c}
        \hline
         Method / top\_k (Llama 3-70B, 10K) & 64 & 128 & 256 & 512 & 1024 \\ \hline
        Quest & 72\% & 90\% & 98\% & \textbf{100\%} & \textbf{100\%} \\ 
        \Sys{}+L14 & 87\% & 88\% & 93\% & \textbf{100\%} & \textbf{100\%}  \\
        \Sys{}+L31 & \textbf{90\%} & \textbf{97\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} \\
        \hline
    \label{tab:llama3-70B-10k}
    \end{tabular}

    \begin{tabular}{c c c c c c c}
        \hline
         Method / top\_k (Llama 3-70B, 32K) & 64 & 128 & 256 & 512 & 1024 \\ \hline
        Quest & 80\% & 88\% & 92\% & 78\% & 95\% \\ 
        \Sys{}+L14 & \textbf{98\%} & 98\% & \textbf{100\%} & \textbf{100\%} & \textbf{100\%}  \\
        \Sys{}+L31 & 82\% & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} \\
        \hline
    \label{tab:llama3-70B-10k}
    \end{tabular}
    
    \begin{tabular}{c c c c c c c}
        \hline
         Method / top\_k (Llama 3-8B, 10K) & 16 & 32 & 64 & 128 & 256 & 512 \\ \hline
        Quest & 70\% & 74\% & 84\% & 99\% & 98\% & \textbf{100\%} \\ 
        \Sys{}+L15 & 74\% & \textbf{92\%} & 88\% & 94\% & 94\% & \textbf{100\%} \\
        \Sys{}+L13 & \textbf{86\%} & 88\% & 98\% & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} \\
        \Sys{}+L9 & 66\% & 90\% & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} \\ \hline
    \label{tab:llama3-8B-10k}
    \end{tabular}

    \vspace{0.5cm}
    
    \begin{tabular}{c c c c c c c}
        \hline
        Method / top\_k (Llama 3-8B, 100K) & 64 & 128 & 256 & 512 & 1024 & 2048 \\ \hline
        Quest & 50\% & 65\% & 87\% & 98\% & \textbf{100\%} & \textbf{100\%} \\ 
        \Sys{}+L15 & 90\% & 92\% & 98\% & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} \\
        \Sys{}+L13 & \textbf{92\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} \\
        \Sys{}+L9 & 70\% & 76\% & 90\% & 96\% & \textbf{100\%} & \textbf{100\%} \\ \hline
    \end{tabular}

    \vspace{0.5cm}

    \begin{tabular}{c c c c c c c}
        \hline
         Method / top\_k (Llama 3.1-8B, 10K) & 16 & 32 & 64 & 128 & 256 & 512 \\ \hline
        Quest & 66\% & 74\% & 86\% & 94\% & \textbf{100\%} & 98\% \\ 
        \Sys{}+L14 & 76\% & 98\% & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} \\
        \Sys{}+L13 & \textbf{84\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} \\ \hline
    \label{tab:llama3.1-8B-10k}
    \end{tabular}

    \vspace{0.5cm}
    
    \begin{tabular}{c c c c c c c}
        \hline
        Method / top\_k (Llama 3.1-8B, 100K) & 64 & 128 & 256 & 512 & 1024 & 2048 \\ \hline
        Quest & \% & \% & \% & \% & \% & \% \\ 
        \Sys{}+L14 & \% & \% & \% & \% & \% & \% \\
        \Sys{}+L13 & \% & \% & \% & \% & \% & \% \\ \hline
    \label{tab:llama3.1-8B-100k}
    \end{tabular}

    \vspace{0.5cm}
    
    \begin{tabular}{c c c c c c}
    \hline
    Method / top\_k (LongChat-7b-v1.5-32k, 10K) & \textbf{32} & \textbf{64} & \textbf{128} & \textbf{256} & \textbf{512} \\
    \hline
    H2O & 0\% & 1\% & 1\% & 1\% & 3\% \\
    TOVA & 0\% & 1\% & 1\% & 3\% & 8\% \\
    StreamingLLM & 1\% & 1\% & 1\% & 3\% & 5\% \\
    Quest & 65\% & \textbf{99\%} & \textbf{99\%} &\textbf{99\%} & \textbf{100\%} \\
    \Sys{}+L7 & \textbf{73\%} & 92\% & 98\% & \textbf{99\%} & \textbf{100\%} \\
    \hline
    \end{tabular}
    
    \vspace{0.5cm}
    
    \begin{tabular}{c c c c c c}
    \hline
    Method / top\_k (Yarn-Llama-2-7b-128k, 100K) & \textbf{256} & \textbf{512} & \textbf{1024} & \textbf{2048} & \textbf{4096} \\
    \hline
    H2O & 2\% & 2\% & 2\% & 2\% & 4\% \\
    TOVA & 2\% & 2\% & 2\% & 2\% & 10\% \\
    StreamingLLM & 1\% & 1\% & 1\% & 2\% & 4\% \\
    Quest & \textbf{88\%} & \textbf{92\%} & \textbf{96\%} & \textbf{100\%} & \textbf{100\%} \\
     \Sys{}+L7 & 58\% & 71\% & 80\% & 84\% & 90\% \\
    \hline
    \end{tabular}
    \caption{(i) Performance of \Sys{} vs. Quest for the 10K-context-length Needle-in-the-Haystack test. (ii) Results for 100K context-length. Both (i) and (ii) are evaluated on gradientai/Llama-3-8B-Instruct-Gradient-1048k. (iii) evaluated with 10k-context-length on LongChat-7b-v1.5-32k; (iv) evaluated with100k-context-length on Yarn-Llama-2-7b-128k; \Sys{}+L$x$ means applying correction at Layer $x$.}
    \label{table:needle_haystack_combined}
\end{table}
 

==> src/figs/scripts/full_heatmaps.tex <==
\begin{figure}[htbp]
    \centering
    % Image 1
    \begin{subfigure}{0.32\textwidth}
        \includegraphics[width=\textwidth]{src/figs/retrieval_heatmaps/256/heatmaps_grouped_256_1891.png}
        \caption{Top-k = 256, Length = 2K}
    \end{subfigure}
    % Image 2
    \begin{subfigure}{0.32\textwidth}
        \includegraphics[width=\textwidth]{src/figs/retrieval_heatmaps/256/heatmaps_grouped_256_9889.png}
        \caption{Top-k = 256, Length = 10K}
    \end{subfigure}
    % Image 3
    \begin{subfigure}{0.32\textwidth}
        \includegraphics[width=\textwidth]{src/figs/retrieval_heatmaps/256/heatmaps_grouped_256_99889.png}
        \caption{Top-k = 256, Length = 100K}
    \end{subfigure}
    \caption{Heatmaps for Top-k = 256 with different lengths.}
    \label{fig:retrieval_heatmaps_256}
\end{figure}



==> src/figs/scripts/partial_heatmap.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.7\textwidth]{src/figs/retrieval_heatmaps/correction/heatmaps_grouped_256_99889.pdf}
    \caption{Retrieval heatmaps for each KV head with top-k = 256, context-length = 100K from layer 3, 12, 21 and 30 with Llama-3-8B-Instruct-Gradient-1048k model on PG19 dataset \cite{raecompressive2019} during generation using top-k sparse attention. Brighter positions represent higher frequency of selection. The tokens are grouped in 1K bins for better illustration. \ref{app:full_retrieval_patter} includes full retrieval patterns for different lengths and top-k.}
    \label{fig:partial_retrieval_heatmaps_256}
\end{figure}

==> src/table/LongBench_old.tex <==
\begin{table}[htbp]
\centering
\caption{Performance across LongBench datasets (Higher is better)}
\renewcommand{\arraystretch}{1.5} % Increase row height for better readability
\begin{tabular}{l|c|c|c|c|c}
\hline
\textbf{Dataset} & \textbf{256} & \textbf{512} & \textbf{1024} & \textbf{2048} & \textbf{4096} \\
\hline
\multicolumn{6}{c}{\textbf{Qasper}} \\
\hline
\textbf{Baseline} & 15.00 & 15.00 & 15.00 & 15.00 & 15.00 \\
\textbf{Quest}    & 11.02 & 12.23 & 12.19 & 13.51 & 13.63 \\
\textbf{\Sys{}}   & 9.63  & 11.62 & 13.43 & 12.89 & 14.09 \\
\hline
\\
\multicolumn{6}{c}{\textbf{NarrativeQA}} \\
\hline
\textbf{Baseline} & 7.36 & 7.36 & 7.36 & 7.36 & 7.36 \\
\textbf{Quest}    & 4.90 & 5.29 & 5.69 & 6.85 & 6.53 \\
\textbf{\Sys{}}   & 10.52 & 9.92 & 10.10 & 8.51 & 6.96 \\
\hline
\\
\multicolumn{6}{c}{\textbf{HotpotQA}} \\
\hline
\textbf{Baseline} & 11.84 & 11.84 & 11.84 & 11.84 & 11.84 \\
\textbf{Quest}    & 9.66  & 10.68 & 10.81 & 11.29 & 10.95 \\
\textbf{\Sys{}}   & 9.81  & 10.84 & 11.77 & 10.71 & 11.72 \\
\hline
\\
\multicolumn{6}{c}{\textbf{MultiFieldQA}} \\
\hline
\textbf{Baseline} & 30.76 & 30.76 & 30.76 & 30.76 & 30.76 \\
\textbf{Quest}    & 18.63 & 23.34 & 26.18 & 26.44 & 28.72 \\
\textbf{\Sys{}}   & 20.61 & 25.20 & 30.33 & 28.89 & 29.61 \\
\hline
\\
\multicolumn{6}{c}{\textbf{GovReport}} \\
\hline
\textbf{Baseline} & 16.77 & 16.77 & 16.77 & 16.77 & 16.77 \\
\textbf{Quest}    & 15.83 & 15.57 & 15.89 & 16.46 & 16.71 \\
\textbf{\Sys{}}   & 15.10 & 15.58 & 16.41 & 16.49 & 16.78 \\
\hline
\\
\multicolumn{6}{c}{\textbf{TriviaQA}} \\
\hline
\textbf{Baseline} & 86.56 & 86.56 & 86.56 & 86.56 & 86.56 \\
\textbf{Quest}    & 74.07 & 80.73 & 83.47 & 84.82 & 85.91 \\
\textbf{\Sys{}}   & 62.12 & 73.96 & 78.31 & 84.26 & 86.95 \\
\hline
\end{tabular}
\end{table}

